A New Wave in Robotics: Survey on Recent mmWave Radar Applications in Robotics

We survey the current state of millimeterwave (mmWave) radar applications in robotics with a focus on unique capabilities, and discuss future opportunities based on the state of the art. Frequency Modulated Continuous Wave (FMCW) mmWave radars operating in the 76--81GHz range are an appealing alternative to lidars, cameras and other sensors operating in the near visual spectrum. Radar has been made more widely available in new packaging classes, more convenient for robotics and its longer wavelengths have the ability to bypass visual clutter such as fog, dust, and smoke. We begin by covering radar principles as they relate to robotics. We then review the relevant new research across a broad spectrum of robotics applications beginning with motion estimation, localization, and mapping. We then cover object detection and classification, and then close with an analysis of current datasets and calibration techniques that provide entry points into radar research.

==> other.tex <==
\keh{Currently this section covers around 6 citations (109-115). It has ample opportunity for expansion if we wish to add more. We have no citations under GPR and only one citation under Marine radar. Alternatively, I think we could consider cutting this section as we had previously discussed.}

\subsection{Synthetic Aperture Radar}
Synthetic aperture radar or SAR is a radar based algorithm which increases the accuracy and resolution of a radar system by correlating signals sent and received across the sensors trajectory, artificially creating a larger antenna or ``aperture" in the process. For an in depth guide on the origin of SAR we refer readers to \cite{tomiyasu1978tutorial} a tutorial on pulsed satellite radar SAR. And for a modern tutorial with MIMO beamforming applications with SAR interferometry (inSAR) we recommend \cite{moreira2013tutorial}. 

Leveraging SAR in robotics applications can be difficult, given the expectation of robust odometry and relatively static environments necessary. However, some researchers have still created novel applications of the technology. 

For instance, \citet{watts20162d} used the robotic arm of a PR2 robot to demonstrate how SAR imaging of objects could be used to accomplished even with centimeter accuracy position estimations based on on-board arm encoders. They showed that 3D point clouds of objects could be generated to assist in object manipulation in the presence of visual obstructions. \figref{fig:sar_spring} demonstrates their method generating a 3D SAR pointcloud of a spring. 

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/sar_spring_watts_2016.PNG}
    \caption{3D SAR image of a spring captured from a mmWave radar attached to a PR2 robotic arm's end-effector presented in \cite{watts20162d}.}
    \label{fig:sar_spring}
\end{figure*}

\citet{yanik2019sar} used a cascaded mmWave radar sensor on a precision two axis scanner to develop accurate 3D SAR images using mmWave radar sensors using an custom explicit near-field MIMO array to convert the multi-static antenna system to a mono-static system for SAR analysis. A SAR image of scissors obscured by a box is shown in Figure \ref{fig:sar_scissors}.

\begin{figure}[htb!]
    \centering
    \begin{tabular}{cc}
    \subfloat[Experiment Setup]{\includegraphics[height=4cm]{figures/sar_scissors_experiment.PNG}\label{fig:sar_scissors_exp}}&
    \subfloat[SAR Image]{\includegraphics[height=4cm]{figures/sar_scissors_results.PNG}\label{fig:sar_scissors_result}}
    \end{tabular}
    \caption{Example experiment from \cite{yanik2019sar} showing a SAR image of scissors obscured by a cardboard box.}
    \label{fig:sar_scissors}
\end{figure}

These applications of SAR could be quite useful in creating intelligent manufacturing robots with radar systems equipped to assist in obstructed manipulation tasks. 

\citet{laribi2018performance} used the Range Migration Algorithm \cite{jin1984sar} for image correlation on a vehicle mounted radar to generate accurate SAR images of static scenes recorded while in motion. This has limited applications in more dynamic environments, but shows the advantages or SAR based imaging resolutions in ideal conditions. Specifically they were able to accurate measure the distances of and between parked vehicles, and identify consistent features of the entryway of a building including stairs, hand rails, and columns surrounding doors. Their work shows potential applications of SAR in mapping, and localization in limited contexts such as vehicle parking. 

\subsection{Marine Radar}

\cite{kim2021robust_marine} fused ship position estimates from cameras conducted by YoloV3 \cite{redmon2018yolov3} and from radar using U-net architecture using a consistency based data association metric, outperforming a strict NN approach to association noisy radar projects to individual ships. 

\subsection{Ground Penetrating Radar}


\subsection{Delphi Radar}
\keh{Have there been attempts to characterize other common sensors e.g. Navtech/TI AWR/Smartmicro UMR?}

\citet{stanislas2015characterisation} conduct a detailed analysis of the effects of various environmental parameters and practical uses of a Delphi scanning radar, characterizing error, changes from the environment, and ability to target useful object in short range robotics applications. 
